Incremental Neural Coreference Resolution in Constant Memory

We investigate modeling coreference resolution under a fixed memory constraint by extending an incremental clustering algorithm to utilize contextualized encoders and neural components. Given a new sentence, our end-to-end algorithm proposes and scores each mention span against explicit entity representations created from the earlier document context (if any). These spans are then used to update the entity's representations before being forgotten; we only retain a fixed set of salient entities throughout the document. In this work, we successfully convert a high-performing model (Joshi et al., 2020), asymptotically reducing its memory usage to constant space with only a 0.3% relative loss in F1 on OntoNotes 5.0.

==> 883 arxiv/algorithms/inference.tex <==
\begin{algorithm}
\small
\caption{FindClusters(Document)}
\label{alg:inference}
\begin{algorithmic}
\State Create an empty Entity List, $E$
\For{segment $\in$ Document}
    \State $M \gets$ \textsc{Spans}$($segment$)$
    \For {$m \in M$}
        \State $scores \gets \textsc{PairScore}(m, E)$
        \State $top\_score \gets \text{max}(scores)$ 
        \State $top\_e \gets \text{argmax}(scores)$
        \If {$top\_score > 0$}
            \State $\textsc{Update}(top\_e, m)$
        \Else
            \State $\textsc{Add\_new\_entity}(E, m)$
        \EndIf
    \EndFor
    \State \textsc{Evict}($E$)
\EndFor
\State \Return $E$
\end{algorithmic}
\end{algorithm}

==> 883 arxiv/figures/clusters_fig.tex <==
\begin{figure*}[ht]
    \centering
    \def\svgwidth{0.97\columnwidth}
    \begin{subfigure}{0.97\columnwidth}
    \vspace{2mm}
        \input{figures/clusters_tex.pdf_tex}
    \end{subfigure}
    \begin{subfigure}{\columnwidth}
    \fbox{
    \parbox{0.93\columnwidth\linespread{1.0}\selectfont}{
        \begin{small}
        \textit{
            President Clinton may travel to North Korea in an attempt to improve relations with that country. The announcement comes after two days of talks between American and North Korean leaders in Washington. Secretary of State Madeleine Albright has accepted an invitation to visit North Korea and meet with leader Kim Jong-il. She made the unexpected announcement at a dinner last night in Washington. North Korea's top defense official hosted the event. The country is on a U.S. list of nations that sponsor terrorism. The Clinton administration is trying to persuade North Korea to halt its ballistic missile program as a way it can get off the list. There's no word yet when Albright's trip will take place.
        }
        \end{small}
        }
    }
    \end{subfigure}
    \caption{t-SNE plot (left) of span representations of a single document (right) in the development set (cnn\_0040\_0). Each color/shape is a predicted cluster, while light gray circles indicate predicted singletons. For each span, the gold cluster label (-1, if not annotated) and its contribution to the entity embedding is noted in parentheses.}
    \label{fig:clusters}
\end{figure*}

==> 883 arxiv/figures/memory_fig.tex <==
\begin{figure}
    \centering
    \def\svgwidth{\columnwidth}
    \input{figures/memory_tex.pdf_tex}
    \caption{Total size of GPU-allocated tensors for each document in the development set. The base (\textbf{JS-B}) and large (\textbf{JS-L}) models of the baseline use apparently linear space, while ours with inference segment lengths of 128 and 512 use constant space.}
    \label{fig:memory}
\end{figure}

==> 883 arxiv/tables/full.tex <==
\begin{table*}[ht!]
    \small
    \centering
    \begin{tabular}{lcccccccccc}
    \toprule
     & \multicolumn{3}{c}{MUC} & \multicolumn{3}{c}{B$^3$} & \multicolumn{3}{c}{CEAF$_{\phi_4}$} & \\
    & P & R & F1 & P & R & F1 & P & R & F1 & Avg. F1\\
    \midrule
     Baseline \cite{joshi2019spanbert} & 85.8 & 84.8 & 85.3 & 78.3 & 77.9 & 78.1 & 76.4 & 74.2 & 75.3 & 79.6\\
     Ours & 85.7 & 84.8 & 85.3 & 78.1 & 77.5 & 77.8 & 76.3 & 74.1 & 75.2 & 79.4\\
     Ours (without eviction) & 85.7 & 84.9 & 85.3 & 78.1 & 77.5 & 77.8 & 76.2 & 74.2 & 75.2 & 79.4\\
     \midrule
    CorefQA \cite{wu-etal-2020-corefqa} & 88.6 & 87.4 & 88.0 & 82.4 & 82.0 & 82.2 & 79.9 & 78.3 & 79.1 & 83.1 \\
    \bottomrule
    \end{tabular}
    \caption{Complete results of our model on the OntoNotes 5.0 test set with three coreference resolution metrics: MUC, B$^3$, and CEAF$_{\phi_4}$. For completeness, we also present the values for the current state-of-the-art. All models use an encoder derived from SpanBERT-large.}
    \label{tab:full}
\end{table*}

==> 883 arxiv/tables/memory.tex <==
\begin{table}[t]
    \small
    \centering
    \begin{tabular}{rcc}
    \toprule
     Model & GPU Memory (GB) & Dev. F1 \\
    \midrule
     Our model & 2.0 & 79.5 \\
     No eviction & 2.0 & 79.7 \\
     \midrule 
     \textbf{JS-B} & 6.4 & 77.7 \\
     \textbf{JS-L} & \textgreater 11.9 & 80.1 \\
     \bottomrule
    \end{tabular}
    \caption{Space needed and performance over the development set. \textbf{JS-B} and \textbf{JS-L} refer to the \texttt{base} and \texttt{large} variants SpanBERT used in the baseline.}
    \label{tab:memory}
\end{table}


==> 883 arxiv/tables/performance.tex <==
\begin{table}[ht]
    \small
    \centering
    \begin{tabular}{rccccr}
    \toprule
     Subset & \#Docs & \textbf{JS-L} & Ours & $\Delta$ & -evict\\
    \midrule
     All & 343 & 80.1 & 79.5 & -0.6 & 79.7\\
     0-128 & 57 & 84.6 & 84.5 & -0.1 & 84.5 \\
     129-256 & 73  & 83.7 & 83.6 & -0.1 & 83.6 \\
     257-512 & 78  & 82.9 & 83.4 & +0.5 & 83.4\\
     513-768 & 71  & 80.1 & 79.3 & -0.8 & 79.3 \\
     769-1152 & 52  & 79.1 & 78.6 & -0.5 & 79.0 \\
     1153+ & 12  & 71.3 & 69.6 & -1.7 & 69.8\\
     \midrule
     1 Speaker & 268 & 81.1 & 81.0 & -0.1 & 81.2\\
     2+ Speakers & 75 & 76.7 & 75.0 & -1.7 & 75.0\\
     \midrule
     Test & 348 & 79.6 & 79.4 & -0.2 & 79.4\\
    \bottomrule
    \end{tabular}
    \caption{Average F1 score on the development set broken down by document length and number of speakers. \textbf{JS-L} refers to the \texttt{spanbert\_large} model from \citet{joshi2019spanbert}, which we treat as our baseline, and -evict refers to the model without eviction.}
    \label{tab:distance}
\end{table}


==> 883 arxiv/tables/segment.tex <==
\addtolength{\tabcolsep}{-3pt}
\begin{table}[ht]
    \small
    \centering
    \begin{tabular}{crcccc}
    \toprule
    & & \multicolumn{4}{c}{Inference Length}\\
     & & \multicolumn{2}{c}{Sentences} & \multicolumn{2}{c}{Tokens} \\
     &Train$\downarrow$ & 1 sent. & 10 sent. & 128 toks. & 512 toks. \\
      \midrule
     \multirow{3}{*}{\rotatebox[origin=c]{90}{sents.}} & 1 & 70.0 & 76.4 & 75.2 & 76.9 \\
     & 5 & 70.0 & 77.4 & 76.4 & 78.6 \\
     & 10 & 68.9 & 77.8 & 76.2 & 78.9\\
     \midrule
     \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{toks.}}} & 128  & 70.1 & 77.2 & 76.3 & 77.7 \\
     & 256  & 69.1 & 77.9 & 76.5 & 78.8 \\
     & 384  & 67.7 & 77.3 & 76.1 & 79.1 \\
     & 512  & 67.1 & 77.7 & 75.6 & 79.7 \\
     \bottomrule
    \end{tabular}
    \caption{Average dev. F1 score for models trained and evaluated across a range of segment lengths (either fixed number of sentences or subtokens).}
    \label{tab:segment}
\end{table}
\addtolength{\tabcolsep}{3pt}
